Parabolic Approximation Line Search for DNNs

A major challenge in current optimization research for deep learning is to automatically find optimal step sizes for each update step. The optimal step size is closely related to the shape of the loss in the update step direction. However, this shape has not yet been examined in detail. This work shows empirically that the batch loss over lines in negative gradient direction is mostly convex locally and well suited for one-dimensional parabolic approximations. By exploiting this parabolic property we introduce a simple and robust line search approach, which performs loss-shape dependent update steps. Our approach combines well-known methods such as parabolic approximation, line search and conjugate gradient, to perform efficiently. It surpasses other step size estimating methods and competes with common optimization methods on a large variety of experiments without the need of hand-designed step size schedules. Thus, it is of interest for objectives where step-size schedules are unknown or do not perform well. Our extensive evaluation includes multiple comprehensive hyperparameter grid searches on several datasets and architectures. Finally, we provide a general investigation of exact line searches in the context of batch losses and exact losses, including their relation to our line search approach.

==> paper_NIPS2020_arxive_v2_2021_10_25 (copy)/commands_neurips_2020.tex <==
\newcommandx{\BL}[1][1=t]{\mathcal{L}_{\mathbb{B}_{#1}}}
%\newcommandx{\BL}[2][1=\space ,2=t]{\mathcal{L}_{\mathbb{B}_{#1},{#2}}}
\newcommandx{\s}[1][1=\space]{s_{\text{upd}_{#1}}}
\renewcommandx{\vec}{\boldsymbol}
\renewcommandx{\mathbf}{\boldsymbol}

==> paper_NIPS2020_arxive_v2_2021_10_25 (copy)/proofs/convergence_proof.tex <==

\begin{proposition_ap}
	PAL converges on  $f : \mathbb{R}^n \rightarrow \mathbb{R}, \mathbf{x} \mapsto c+\mathbf{r}^T\mathbf{x}+\mathbf{x}^T\mathbf{Q}\mathbf{x}$ with $\mathbf{Q}\in \mathbb{R}^{n\times n}$ hermitian and positive definite.
\end{proposition_ap}
%\vspace{-0.5cm}
%\small
%\doublespacing
\begin{proof}
	\quad
\\For this prove we consider a basic \pal\ without the features introduced in Section \ref{subsec:features}.
Note, that during the proof we will see, that $a>0$ and $b<0$. Thus, only the update step for this case has to be considered (see Section \ref{subsec:casediscrimination}.
	
 \quad \\ 
 $f(\mathbf{x})$ is convex since $\mathbf{Q}$ is positive definite. Thus it has one minimum.\\
 Without loss of generality we set $c=0,\mathbf{r}=\mathbf{0},\mathbf{x}_n \neq 0$ %since the optimization problem does not change when the minimum location is moved to the origin and its value is set to 0. \\We get:
 \begin{equation}
 f(\mathbf{x})=\mathbf{x}^T\mathbf{Q}\mathbf{x} \text{ and }\nabla_{\mathbf{x}} f(\mathbf{x})= f'(\mathbf{x})=2\mathbf{Q}\mathbf{x}
   \end{equation}
The values of $f(x)$ along a line through $\mathbf{x}$ in the direction of $-f'(\mathbf{x})$ are given by:
 \begin{equation}
 f(-f'(\mathbf{x})\hat{s}+\mathbf{x})
   \end{equation}   
%The update step  $\hat{s}_{min}$ to the minimum of the line is:
%\begin{equation}
%\hat{s}_{min}= \argmin{\hat{s}} f(-f'(\mathbf{x}_n)\hat{s}+\mathbf{x}_n)
%\end{equation}
 %We set $s_{upd}=s_{min}||f'(x_n)||$ to simplify the further steps. $||f'(x_n)|| > 0$ since otherwise we would already be in the extremum. Note that $f(\mathbf{x})$ is convex.\\
 %Note that $f(-f'(\mathbf{x}_n)\hat{s}+\mathbf{x}_n)= a\hat{s}^2+b\hat{s}+c$ since $f(\mathbf{x})$ is an $n$ dimensional parabolic function and the values along each line of $f(\mathbf{x})$ are a parabolic function again. $a > 0$ since $\mathbf{Q}$ is positive definite.\\
Now we expand the line function:
\begin{equation}
\begin{aligned}
f(-f'(\mathbf{x})\hat{s}+\mathbf{x})&=
f(-2\mathbf{Q}\mathbf{x}\hat{s}+\mathbf{x})\\&=(-2\mathbf{Q}\mathbf{x}\hat{s}+\mathbf{x})^T\mathbf{Q}(-2\mathbf{Q}\mathbf{x}\hat{s}+\mathbf{x})
\\&=\underbrace{4\mathbf{x}^T\mathbf{Q}^3\mathbf{x}}_{=:a}\hat{s}^2+\underbrace{-4\mathbf{x}^T\mathbf{Q}^2\mathbf{x}}_{=:b}\hat{s}+\underbrace{\mathbf{x}^T\mathbf{Q}\mathbf{x}}_{=:c}
\end{aligned}
\end{equation}
 \\ Here we see that $f(\hat{s})$ is indeed a parabolic function with $a>0$, $b<0$ and $c>0$ since $\mathbf{Q}^3$, $\mathbf{Q}^2$ and $\mathbf{Q}$ are positive definite.\\
The location of the minimum $s_{min}$ of $f(\hat{s})$ is given by:
\begin{equation}
	 \hat{s}_{min}=\argmin{\hat{s}} f(-f'(\mathbf{x})\hat{s}+\mathbf{x})=-\frac{b}{2a}
\end{equation}
 \pal\ determines $\hat{s}_{min}$ exactly with $\hat{s}_{min}=\frac{s_{upd}}{||f'(x)||}$ (see equation 1 and 2). $||f'(x)||>0$  since otherwise we are already in the minimum.\\

\noindent The value at the minimum is given by: 
\begin{equation}
f(\hat{s}_{min})\\= a(\frac{-b}{2a})^2+b(\frac{-b}{2a})+c\\=-\frac{b^2}{4a}+c\\
%=-\frac{(4\mathbf{x}^T\mathbf{Q}^2\mathbf{x})^2}{16\mathbf{x}^T\mathbf{Q}^3\mathbf{x}}+\mathbf{x}^T\mathbf{Q}\mathbf{x}
=-\underbrace{\frac{(-\mathbf{x}^T\mathbf{Q}^2\mathbf{x})^2}{\mathbf{x}^T\mathbf{Q}^3\mathbf{x}}}_{=:g(\mathbf{x})}+\mathbf{x}^T\mathbf{Q}\mathbf{x}
\\=-g(\mathbf{x})+f(\mathbf{x}) \\
\end{equation}
Since $\mathbf{Q}^2$ and $\mathbf{Q}^3$ are positive definite and $\mathbf{x}\neq 0$: \begin{equation}g(\mathbf{x})>0\end{equation}
% Since $f(\mathbf{x})$ is positive we have:\\
% \begin{equation} 0<f(\mathbf{x}_{n+1})<f(\mathbf{x}_{n})<\ldots<f(\mathbf{x}_{0})
% \end{equation}
Now we consider the sequence $f(\mathbf{x}_n)$, with $\mathbf{x}_n$ defined by \textit{PAL} (see Equation 1): \\
\begin{equation}
\mathbf{x}_{n+1}=-\frac{f'(\mathbf{x}_n)}{||f'(x_n)||}\hat{s}_{upd}+\mathbf{x}_n= -f'(\mathbf{x}_n)\hat{s}_{min}+\mathbf{x}_n
\end{equation}
 It is easily seen by induction that:
 \begin{equation}
  0<f(\mathbf{x}_{n+1})<f(\mathbf{x}_{n})=\sum\limits_{i=0}^{n-1} -g(\mathbf{x}_i) +f(\mathbf{x}_0)< f(\mathbf{x}_0). 
\end{equation}
  $g(\mathbf{x}_{n})$ converges to 0. Since $\forall n:g(\mathbf{x_n})>0$ and $\sum\limits_{i=0}^{n-1} -g(\mathbf{x}_i)$ is bounded. \\
  \\ Now we have to show that $\mathbf{x}_n$ converges to 0.
 \\ We have:
  \begin{equation}
  g(\mathbf{x}_n)=\frac{(\mathbf{x}_n^T\mathbf{Q}^2\mathbf{x}_n)^2}{\mathbf{x}_n^T\mathbf{Q}^3\mathbf{x}_n}=\frac{\langle\mathbf{x}_n,\mathbf{Q}^2\mathbf{x}_n\rangle^2}{\langle\mathbf{x}_n,\mathbf{Q}^3\mathbf{x}_n\rangle}
  \end{equation}
 Now we use the theorem of Courant-Fischer:
   \begin{equation}
   \begin{aligned}
   \langle x,x\rangle\min\{\lambda_1,\dots,\lambda_n\}\leq \langle x,Ax \rangle\leq \langle x,x \rangle \max\{\lambda_1,\dots,\lambda_n\}\\ \text{ for any symmetric }  A \in \mathbb{R}^{n\times n} \text{ with } \lambda_1,\dots,\lambda_n
      \end{aligned}
   \end{equation}
    And get: 
\begin{equation}
g(\mathbf{x}_n) \geq \frac{\lambda^2_{\mathbf{Q}^2\min} \langle \mathbf{x}_n,\mathbf{x}_n \rangle^2}{\lambda_{\mathbf{Q}^3\max} \langle \mathbf{x}_n,\mathbf{x}_n \rangle}=C \frac{||\mathbf{x}_n||^4}{||\mathbf{x}_n||^2}=C ||\mathbf{x}_n||^2
\end{equation} 
with \begin{equation}C=\frac{\lambda^2_{\mathbf{Q}^2\min}}{\lambda_{\mathbf{Q}^3\max}}>0 \text{ since all } \lambda \text{ of the positive definite } \mathbf{Q} \text{ are positive} \end{equation}
 Thus, we have:
\begin{equation}
 g(\mathbf{x}_n) \geq C ||\mathbf{x}_n||^2 \geq 0 \end{equation} 
 Since $g(\mathbf{x}_n)$ converges to 0,  $C ||\mathbf{x}_n||^2 $ converges to 0. \\This means, $\mathbf{x}_n$ converges to $\mathbf{0} $, which is the location of the minimum. 
\end{proof}
\singlespacing
\normalsize

 
%\end{document}


==> paper_NIPS2020_arxive_v2_2021_10_25 (copy)/proofs/line_proof.tex <==
\begin{lemma_ap}
	Let $f: \mathbb{R}^n \rightarrow \mathbb{R}$ be a k-times continuously differentiable function. Furthermore, assume there exists $a,b,c \in \mathbb{R}$ with $a>0$, such that $f(\mathbf{l}+\mathbf{d}s)= as^2+bs+c$ for all $s \in \mathbb{R}$. Then there exist $z \in \mathbb{R}, \mathbf{r} \in \mathbb{R}^n$ and a positive definite Matrix $\mathbf{Q}\in \mathbb{R}^{n\times n}$ such that $f(\mathbf{x})= c+\mathbf{r}^T\mathbf{x}+\mathbf{x}^T\mathbf{Q}\mathbf{x}$ for all $\mathbf{x} \in \mathbb{R}^n$.
	%f(\mathbf{x})= %c+\mathbf{r}^T\mathbf{x}+\mathbf{x}^T\mathbf{Q}\mathbf{x}$ with $\mathbf{Q}\in %\mathbb{R}^{n\times n}$ hermitian and positive definite.
\end{lemma_ap}
%\vspace{-0.5cm}
%\small
%\doublespacing
\begin{proof}
%	$f(\mathbf{x})$ has the form:\\
\begin{equation}
\begin{aligned}
 g(\mathbf{x})= u+\mathbf{v}^T\mathbf{x}+\mathbf{x}^T\mathbf{W}\mathbf{x} \text{ for some } u\in \mathbb{R}, \mathbf{v}\in \mathbb{R}^n \text{ and } \mathbf{W} \in \mathbb{R}^{n\times n} \\ \Leftrightarrow \forall \mathbf{l},\mathbf{d} \in \mathbb{R}^n \land ||\mathbf{d}||=1 : \sum\limits_{j=1}^{n}\sum\limits_{k=1}^{n}\sum\limits_{l=1}^{n} \frac{\partial^3 g(\mathbf{l}) }{\partial x_j,\partial x_k,\partial x_l}d_{j}d_{k}d_{l}=0
 \end{aligned}
\end{equation}
$\Rightarrow$ holds since we have a polynomial of degree 2 and its third derivative is always a $\mathbf{0}$ tensor.\\
%$\Leftarrow$ holds since the right part is the fourth element of the multivariate Taylor series. Since this element is 0 the following are also 0. The first 3 elements can at most describe a polynomial of degree 3.\\
$\Leftarrow$ holds since the reminder of the quadratic Taylor expansion is always 0.


%$g(\mathbf{x}): for some $u\in \mathbb{R}$,$\mathbf{v}\in \mathbb{R}^n$ and $\mathbf{W} \in \mathbb{R}^{n\times n}$\\
\noindent
In our case the right part is 0 since:
	\begin{equation}
\sum\limits_{j=1}^{n}\sum\limits_{k=1}^{n}\sum\limits_{l=1}^{n} \frac{\partial^3 f(\mathbf{l}) }{\partial x_j,\partial x_k,\partial x_l}d_{j}d_{k}d_{l}= \frac{\partial}{\partial s^3}f(\mathbf{l}+\mathbf{d}s)=0
	\end{equation}
\\	
 In words: $f(\mathbf{x})$ is a parabolic function if and only if for each location $\mathbf{l}$ the third directional derivative of $f(\mathbf{\mathbf{l}})$ in each direction $\mathbf{d}$ is $0$. Which is the case, since the third derivative of each intersection is 0.
\\
$\mathbf{W}$ is positive definite since: \\
%\begin{equation}
%\forall \mathbf{d},\mathbf{l} \in \mathbb{R}^n \land ||\mathbf{d}||=1: a= \frac{1}{2} \frac{\partial}{\partial s^2}f(\mathbf{l}+\mathbf{d}s)=\frac{1}{2}\mathbf{d}^T \mathbf{H}(\mathbf{l}) \mathbf{d} = \mathbf{d}^T \mathbf{W} \mathbf{d} > 0
%\end{equation}
\begin{equation}
\forall \mathbf{d},\mathbf{l} \in \mathbb{R}^n \land ||\mathbf{d}||=1: \mathbf{d}^T \mathbf{W} \mathbf{d} =\frac{1}{2}\mathbf{d}^T \mathbf{H}(\mathbf{l}) \mathbf{d}= \frac{1}{2} \frac{\partial}{\partial s^2}f(\mathbf{l}+\mathbf{d}s) = a > 0
\end{equation}
where $\mathbf{H}$ is the Hessian.
\end{proof}

==> paper_NIPS2020_arxive_v2_2021_10_25 (copy)/proofs/minimum_proof.tex <==
\begin{proposition}
	If $ \mathcal{L}(\mathbf{\theta}) : \mathbb{R}^n \rightarrow \mathbb{R}$ $\mathbf{\theta} \mapsto  \mathcal{L}(\mathbf{\theta})=\frac{1}{m}\sum_{i=1}^m c_i+\mathbf{r}_i^T\mathbf{\theta}+\mathbf{\theta}^T\mathbf{Q}_i\mathbf{\theta}$ and $ c_i+\mathbf{r}_i^T\mathbf{\theta}+\mathbf{\theta}^T\mathbf{Q}_i\mathbf{\theta}= \BL[i](\mathbf{\theta})$ with $m$ being number the of batches $\mathbb{B}_i$. (Each batch defines a parabola. The empirical loss $\mathcal{L}(\mathbf{\theta})$ is the mean of these parabolas). And for all  $i,j \in \mathbb{N}$ it holds that $ \mathbf{Q}_i=\mathbf{Q}_j$ and that $\mathbf{Q_i}$ is positive definite. Then $\argmin{\theta} \mathcal{L}(\mathbf{\theta}) =\frac{1}{m}\sum_{i=1}^m\argmin{\theta} \BL[i](\mathbf{\theta})$ holds.
\end{proposition}

\begin{proof}
 \quad\\ 
 Since $\mathcal{L}(\mathbf{\theta})$ is a sum of convex functions, it is also convex and has one minimum.\\
 At first we determine the derivative of $\mathcal{L}(\mathbf{\theta})$ with respect to $\mathbf{\theta}$:
  \begin{equation}
 \frac{\partial}{\partial \mathbf{\theta}}\mathcal{L}(\mathbf{\theta})= \frac{1}{m}\sum\limits_{i=1}^m(\mathbf{r}_i+2\mathbf{Q}_i\mathbf{\theta})= 2\mathbf{Q}\mathbf{\theta}+\frac{1}{m}\sum\limits_{i=1}^m\mathbf{r}_i
 \end{equation}
% Let: 
% \begin{equation}
% 	\begin{aligned}
% 	\hat{\mathbf{\theta}} &= \argmin{\mathbf{\theta}} \mathcal{L}(\mathbf{\theta})\\
% 	\hat{\mathbf{t}} &= \argmin{\mathbf{t}} L(\mathbf{t})
% 	 \end{aligned}
% \end{equation}
Then we determine the minima:
   \begin{equation}
  \argmin{\mathbf{\theta}} \mathcal{L}(\mathbf{\theta}) \Leftrightarrow
 \frac{\partial}{\partial \mathbf{\theta}}\mathcal{L}(\mathbf{\theta}){=}\mathbf{0} \Leftrightarrow \mathbf{\theta}=-\frac{1}{2}( \sum\limits_{i=1}^m \mathbf{Q}_i)^{-1} \sum\limits_{i=1}^m \mathbf{r_i}= -\frac{1}{2m} \mathbf{Q}^{-1} \sum\limits_{i=1}^m \mathbf{r_i}
   \end{equation}
   \begin{equation}
\argmin{\mathbf{\theta}} \BL[i](\mathbf{\theta})=-\frac{1}{2}\mathbf{Q}^{-1}\mathbf{r}_i
 \end{equation}
 Thus, we get:
 \begin{equation}
  \argmin{\mathbf{\theta}} \mathcal{L}(\mathbf{\theta})= -\frac{1}{2m}\mathbf{Q}^{-1}\sum\limits_{i=1}^m \mathbf{r}_i=\frac{1}{m}\sum\limits_{i=1}^m -\frac{1}{2}\mathbf{Q}^{-1}\mathbf{r}_i =\frac{1}{m}\sum\limits_{i=1}^m\argmin{\mathbf{\theta}} \BL[i](\mathbf{\theta})
  \end{equation}
\end{proof}
